Vote from the Center: 6 DoF Pose Estimation in RGB-D Images by Radial Keypoint Voting

We propose a novel keypoint voting scheme based on intersecting spheres, that is more accurate than existing schemes and allows for fewer, more disperse keypoints. The scheme is based upon the distance between points, which as a 1D quantity can be regressed more accurately than the 2D and 3D vector and offset quantities regressed in previous work, yielding more accurate keypoint localization. The scheme forms the basis of the proposed RCVPose method for 6 DoF pose estimation of 3D objects in RGB-D data, which is particularly effective at handling occlusions. A CNN is trained to estimate the distance between the 3D point corresponding to the depth mode of each RGB pixel, and a set of 3 disperse keypoints defined in the object frame. At inference, a sphere centered at each 3D point is generated, of radius equal to this estimated distance. The surfaces of these spheres vote to increment a 3D accumulator space, the peaks of which indicate keypoint locations. The proposed radial voting scheme is more accurate than previous vector or offset schemes, and is robust to disperse keypoints. Experiments demonstrate RCVPose to be highly accurate and competitive, achieving state-of-the-art results on the LINEMOD 99.7% and YCB-Video 97.2% datasets, notably scoring +4.9% higher 71.1% than previous methods on the challenging Occlusion LINEMOD dataset, and on average outperforming all other published results from the BOP benchmark for these 3 datasets. Our code is available at http://www.github.com/aaronwool/rcvpose.

==> DvsScaleTable.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}[t]
%   \resizebox{\columnwidth}{!}{%
\begin{center}
\begin{tabular}
%   {|c|c|c|c|c|c|}
{rccccc}
\hline
scale factor & 1 & 2 & 3 & 4 & 5 \\ \hline
%   $\mu$ [mm]& .79 & .65 & .62 & .61 & .61 \\ \hline
%   $\sigma$ [mm] & .17 & .19 & .20 & .21 & .22 \\
$\mu$ [mm]& .93 & .78 & .76 & .75 & .75 \\ \hline
$\sigma$ [mm] & .23 & .24 & .25 & .25 & .25 \\
\hline
\end{tabular}
\end{center}
%   } % \resizebox
\caption{Point Distance Error by Scale Factor: Mean $\mu$ and standard deviation $\sigma$ of distance between ape object points transformed using randomly perturbed keypoints (1.5 mm magnitude), under various keypoint scaling factors.}
\label{tab:DvsScale}
\end{table}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{center}
\begin{tabular}
%   {|c|c|c|c|c|c|}
{rrrrrr}
\cline{2-6} \\[-10pt]
\multicolumn{1}{c}{} &
\multicolumn{5}{c}{point distance error mean (standard deviation) [mm]} \\ 
\hline
\multicolumn{1}{r}
% {\diagbox{object}{scale}} & 
{scale} &
\multicolumn{1}{c}{1} & 
\multicolumn{1}{c}{2} & 
\multicolumn{1}{c}{3} & 
\multicolumn{1}{c}{4} & 
\multicolumn{1}{c}{5} 
\\ \hline
%   $\mu$ [mm]& .79 & .65 & .62 & .61 & .61 \\ \hline
%   $\sigma$ [mm] & .17 & .19 & .20 & .21 & .22 \\
ape& .93 (.23) & .78 (.24) & .76 (.25) & .75 (.25) & .75 (.25) \\ %   \hline
can & .99 (.24) & .79 (.25) & .78 (.29) & .78 (.27) & .75 (.28) \\ 
%   \hline
cat & .89 (.22) & .76 (.27) & .74 (.27)  & .73 (.27) & .72 (.29) \\  
%   \hline
driller & .90 (.23) & .78 (.27) & .75 (.27)  & .75 (.28) & .75 (.28)  \\ 
%   \hline
duck & 1.13 (.34) & .93 (.29) & .91 (.32) & .87 (.37) & .84 (.37) \\ 
%   \hline
eggbox & .86 (.22) & .73 (.24) & .70 (.26) & .69 (.26) & .69 (.27) \\ 
%   \hline
glue & .90 (.23) & .78 (.24) & .76 (.27) & .75 (.27) & .75 (.26) \\ 
%   \hline
holepunch & .97 (.28) & .89 (.29) & .89 (.32) & .86 (.31)  & .82 (.32) \\ 
\hline
%   $\sigma$ [mm] & .23 & .24 & .25 & .25 & .25 \\
\end{tabular}
\end{center}
} % \resizebox
\caption{Point Distance Error for Scaled Keypoints: Mean (standard deviation) in mm of distance between object points transformed with $T$ and $\widetilde{T}$, using keypoints scaled by a radius factor and perturbed with random  1.5 mm magnitude error.}
\label{tab:DvsScale}
\end{table}

==> NumberOfSkipConnections.tex <==
\noindent{\bf Number of Skip Connections: }
There were five different  network
architectures proposed in the intial ResNet paper~\cite{2015Resnet}. 
While some 6 DoF pose recovery works use 
variations of ResNet-18~\cite{pvnet,wang2019densefusion,zakharov2019dpod,trabelsi2021ppn}
others use ResNet-50~\cite{wang2020self6d,Park2020NOL}.
Some customize the structure by converting it to encoder~\cite{trabelsi2021ppn,Park2020NOL,zakharov2019dpod,wang2019densefusion}, adding extra layers and skip connections~\cite{pvnet} while others use the original ResNet unaltered~\cite{PVN3d,park2019pix2pose}. 

We conducted an experiment which 
examined the impact of
the number of skip connections
on mean keypoint estimation error
$\bar{\epsilon}$.
We
increased the 
number of skip connections
for ResNet-18,
from 3 to 5.
Skip connections
improve the influence of image features
during upsampling,
as illustrated in 
Fig.~\ref{fig:pvVsRCV}.
The results are displayed in 
Table~\ref{tab:skipVariation},
and show that increasing 
the skip connections from
3 to 5, decreased 
both the mean
and the stanand Radial Voting
dard deviation 
of the keypoint 
estimation error by a large margin,
in all cases.
\input{tab-SkipVariation}

==> ResNetDepth.tex <==
\noindent{\bf ResNet Depth: }
A further experiment
tested different ResNet depths,
from 18 to 152 layers.
The results are 
plotted in
Fig.~\ref{fig:resnet-depth-plot},
and indicate that the
substantially deeper networks
exhibit only 
a minor reduction in
$\bar{\epsilon}$.

Despite the rather minor improvement
due to increased depth,
we nevertheless used ResNet-152
with 5 skip connections
in the RCVPose in our experiments.
It is likely that we would have received
very similar results had we based
our backbone network on ResNet-18,
albeit with a faster training cycle and
smaller memory footprint.

%   \input{tab-ResnetVariation}


\input{fig-resnetDepthPlot}

==> fig-NKeyptsPlot.tex <==
\begin{figure}[t]
\begin{center}
  % \includegraphics[width=0.9\textwidth]{plot-1.png}
%\vspace{-0.5 cm}
%   \hspace{-1.1 cm}
\includegraphics[width=1.0\columnwidth]{plot-NKeypts.pdf}
  \caption{Pose estimation accuracy [mm] vs. number of keypoints}
  \label{fig:NKeyPtsPlot}
\end{center}
%\vspace{-0.5\baselineskip}
\end{figure}

==> fig-depthCorrection.tex <==
\begin{figure}[t]
\begin{center}
  % \includegraphics[width=0.9\textwidth]{plot-1.png}
\includegraphics[width=\columnwidth]{DepthCorrection.png}
  \caption{LineMOD Depth Correction: The projected 3d points aligns better with the model(white points) applied with ground-truth pose by using generated depth(red points) compared to original LindMOD depth sensed by Kinect(pink points)}
  \label{fig:depthCorrection}
\end{center}
\end{figure}

==> fig-dispersionOccLINEMOD.tex <==
\begin{figure}[t]
\begin{center}
%   \includegraphics[width=0.9\textwidth]{plot-1.png}
\includegraphics[width=0.8\columnwidth]{occlinemodDispersionTest.png}
  \caption{Keypoint Dispersion ADD(s) Test on Occlusion LINEMOD: The average ADD(s) precision of $2 \times$ dispersed keypoint performs the best among all four dispersion level}
  \label{fig:dispersionOccLINEMOD}
\end{center}
\end{figure}

==> fig-radialVoting2D.tex <==
\begin{figure}[t]
\begin{center}
  % \includegraphics[width=0.9\textwidth]{plot-1.png}
%\includegraphics[width=0.6\columnwidth]{radial-voting-2D.png}
\includegraphics[width=0.5\columnwidth]{radial-voting-2D-rev6.png}
  \caption{Radial voting for points $p_{1}$, $p_{2}$ and $p_{3}$, illustrated as a 2D slice of 3D accumulator space. Forward inference through the network  returns radius values $r_{1}$, $r_{2}$ and $r_{3}$. Accumulator voxels that intersect with all inscribed spheres are incremented, with the global peak of 3 occuring at that voxel containing keypoint $k$}
%   for every $p_i$ that falls on the imaged object.

  \label{fig:radialVoting2D}
\end{center}
%\vspace{-1.5\baselineskip}
\end{figure}

==> fig-test.tex <==


\begin{figure*}[th]
\begin{center}
  \includegraphics[width=0.5\textwidth]{test.pdf}
  \caption{RCVPose system architecture}
  \label{fig:test}
\end{center}
\end{figure*}

==> fig-train.tex <==
\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.5\textwidth]{train&test.pdf}
  \caption{Train.}
  \label{fig:train}
\end{center}
\end{figure*}



==> tab-1+2-rev1.tex <==
\subfloat[LINEMOD (LM) and Occlusion LINEMOD (O-LM) accuracy results.\label{tab:LINEMOD+OccLINEMOD}
% Non-symmetric objects are evaluated with ADD, and
% symmetric objects
% (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
]{
% \begin{tabular}
% {
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{table}[t]
%   \begin{center}
%\resizebox{\columnwidth}{!}{%
%   \resizebox{.75\columnwidth}{!}{%
\begin{tabular}{llcc}
\cline{3-4}
\multicolumn{2}{c}{} &
\multicolumn{2}{c}{ADD(s) [$\%$]} \\
\hline
Mode      & Method    
& LM & O-LM
\\\hline %\hline
&  SSD6D~\cite{kehl2017ssd} & 9.1 & - \\ % \cline{2-4}
& Oberweger~\cite{oberweger2018making}  & - & 27.1 \\% \cline{2-4} 
& Hu et al.~\cite{hu2019segmentation} & - & 30.4 \\% \cline{2-4} 
& Pix2Pose~\cite{park2019pix2pose}  & 72.4  & 32.0 \\% \cline{2-4} 
& DPOD~\cite{zakharov2019dpod}      & 83.0 & 32.8 \\% \cline{2-4} 
& PVNet~\cite{pvnet}      & 86.3 & 40.8 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& DeepIM~\cite{li2018deepim} & 88.6 & - \\ %\cline{2-4}
& PPRN~\cite{trabelsi2021ppn}    & 93.9     & 58.4 \\\hline%\hline
 & YOLO6D~\cite{yolo6d}      & 56.0 & 6.4  \\%\cline{2-4} 
 & SSD6D+ref~\cite{kehl2017ssd} & 34.1 & 27.5 \\%\cline{2-4} 
                              
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & - & 24.9 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 95.2 & 47.3 \\\hline%\hline
& DenseFusion~\cite{wang2019densefusion}        & 94.3 &  - \\%\cline{2-4} 
& PVN3D~\cite{PVN3d}      & 99.4  & 63.2 \\%\cline{2-4} 
& RCVPose     & 99.4 & 70.2 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-4}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 99.7} & {\bf 71.1}\\ \hline
\end{tabular}
%} % \resizebox
%   \end{center}
%\vspace{-0.5\baselineskip}
% \caption{LINEMOD (LM) and Occlusion LINEMOD (O-LM) accuracy results.\label{tab:LINEMOD+OccLINEMOD}
% % Non-symmetric objects are evaluated with ADD, and
% % symmetric objects
% % (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
% }
% %\vspace{-1\baselineskip}
%   \end{table}
  }
% \end{tabular}
% }
\subfloat[YCB-Video accuracy results.\label{tab:ycbvideo}]{

% \begin{table}[ht]
% \begin{center}
%\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{clcc}
\hline  
\begin{tabular}{c} %\vspace{-3 pt} 
Ref? 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt} 
Method 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt}
%   \overline{\mbox{ADD(s)} [$\%$]}
\mbox{ADD(s)} % [$\%$]
\end{tabular} 
&
\begin{tabular}{c} %\vspace{-3 pt}
% \overline{\mbox{AUC} [$\%$]} 
\mbox{AUC} % [$\%$]
\end{tabular} 
\\ [3pt]
\hline%\hline
\multicolumn{1}{c}{{}}                          & {PoseCNN~\cite{posecnn} } 
& 59.9 &  75.8
\\ %\cline{2-4} 
\multicolumn{1}{c}{{}}                              & {DF (per-pixel)~\cite{wang2019densefusion}}  
& 82.9 & 91.2
\\%  \cline{2-4} 
\multicolumn{1}{c}{{}} & {PVN3D~\cite{PVN3d}}
& 91.8 & 95.5
\\ % \cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{No}}     & RCVPose                              
 & \textbf{95.2} & \textbf{96.6}
 \\ \hline%  \hline
\multicolumn{1}{c}{}                          & PoseCNN~\cite{posecnn} 
& 85.4 & 93.0
\\ % \cline{2-4} 
 \multicolumn{1}{c}{}                          & {DF (iterative)~\cite{wang2019densefusion}} 
 & 86.1 & 93.2
 \\ %\cline{2-4} 
\multicolumn{1}{c}{}                          & {PVN3D~\cite{PVN3d}+ICP} 
& 92.3 & 96.1
\\ %\cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{Yes}}     & RCVPose+ICP                         
 & \textbf{95.9} & \textbf{97.2}
 \\ \hline
\end{tabular}
%\end{adjustbox}
%%\vspace{-0.5\baselineskip}
%\vspace{+0.1\baselineskip}
% \caption{YCB-Video accuracy results.\label{tab:ycbvideo}}
% \end{center}
% %\vspace{-2\baselineskip}
% \end{table}
}

==> tab-1+2.tex <==
\begin{table}[t]
\small
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[c]{.5\linewidth}
\centering
\begin{tabular}{llcc}
\cline{3-4}
\multicolumn{2}{c}{} &
\multicolumn{2}{c}{ADD(s) [$\%$]} \\
\hline
Mode      & Method    
& LM & O-LM
\\\hline %\hline
&  SSD6D~\cite{kehl2017ssd} & 9.1 & - \\ % \cline{2-4}
& Oberweger~\cite{oberweger2018making}  & - & 27.1 \\% \cline{2-4} 
& Hu et al.~\cite{hu2019segmentation} & - & 30.4 \\% \cline{2-4} 
& Pix2Pose~\cite{park2019pix2pose}  & 72.4  & 32.0 \\% \cline{2-4} 
& DPOD~\cite{zakharov2019dpod}      & 83.0 & 32.8 \\% \cline{2-4} 
& PVNet~\cite{pvnet}      & 86.3 & 40.8 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& DeepIM~\cite{li2018deepim} & 88.6 & - \\ %\cline{2-4}
& PPRN~\cite{trabelsi2021ppn}    & 93.9     & 58.4 \\\hline%\hline
 & YOLO6D~\cite{yolo6d}      & 56.0 & 6.4  \\%\cline{2-4} 
 & SSD6D+ref~\cite{kehl2017ssd} & 34.1 & 27.5 \\%\cline{2-4} 
                              
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & - & 24.9 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 95.2 & 47.3 \\\hline%\hline
& DenseFusion~\cite{wang2019densefusion}        & 94.3 &  - \\%\cline{2-4} 
& PVN3D~\cite{PVN3d}      & 99.4  & 63.2 \\%\cline{2-4} 
& RCVPose     & 99.4 & 70.2 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-4}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 99.7} & {\bf 71.1}\\ \hline
\end{tabular}
% \label{tab:LINEMOD+OccLINEMOD}
\end{minipage}
 %%%%%%%%%%%%%%%%%%%%%%%%%%
% \hspace{.5\linewidth}
% \raisebox{2 cm}{
% %\vspace{-10 cm}
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[t]{.5\linewidth}
\centering
\begin{tabular}{clcc}
\hline  
\begin{tabular}{c} %\vspace{-3 pt} 
Ref? 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt} 
Method 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt}
%   \overline{\mbox{ADD(s)} [$\%$]}
\mbox{ADD(s)} % [$\%$]
\end{tabular} 
&
\begin{tabular}{c} %\vspace{-3 pt}
% \overline{\mbox{AUC} [$\%$]} 
\mbox{AUC} % [$\%$]
\end{tabular} 
\\ [3pt]
\hline%\hline
\multicolumn{1}{c}{{}}                          & {PoseCNN~\cite{posecnn} } 
& 59.9 &  75.8
\\ %\cline{2-4} 
\multicolumn{1}{c}{{}}                              & {DF (per-pixel)~\cite{wang2019densefusion}}  
& 82.9 & 91.2
\\%  \cline{2-4} 
\multicolumn{1}{c}{{}} & {PVN3D~\cite{PVN3d}}
& 91.8 & 95.5
\\ % \cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{No}}     & RCVPose                              
 & \textbf{95.2} & \textbf{96.6}
 \\ \hline%  \hline
\multicolumn{1}{c}{}                          & PoseCNN~\cite{posecnn} 
& 85.4 & 93.0
\\ % \cline{2-4} 
 \multicolumn{1}{c}{}                          & {DF (iterative)~\cite{wang2019densefusion}} 
 & 86.1 & 93.2
 \\ %\cline{2-4} 
\multicolumn{1}{c}{}                          & {PVN3D~\cite{PVN3d}+ICP} 
& 92.3 & 96.1
\\ %\cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{Yes}}     & RCVPose+ICP                         
 & \textbf{95.9} & \textbf{97.2}
 \\ \hline
\end{tabular}
\end{minipage}
% } %\raisebox
\end{table}

==> tab-4+5.tex <==
\begin{table}
\small
\begin{minipage}[t]{.55\linewidth}
% \parbox{.5\columnwidth}{
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
% \begin{center}
% %\resizebox{\columnwidth}{!}{
\caption{\small Accumulator space resolution $\rho$ [mm] impact on accuracy $\bar{\epsilon}$ [mm], ADD [$\%$], processing speed [fps], and memory [Mbyte], for LINEMOD ape test images. The processing speed includes only the accumulator space time performance. 
\label{tab:tab4}}
%\vspace{\baselineskip}
\begin{tabular}{c|c|c|c|c|l}
\hline
$\rho$  & \multicolumn{2}{c|}{$\bar{\epsilon}$ [mm]}  & ADD & speed   &   \multicolumn{1}{|c}{memory}    \\ %   \cline{2-3}
{[mm]} & $\mu_r$   & $\sigma_r$ &[\%]   & [fps]    &    \multicolumn{1}{|c}{[Mbyte]}    \\ 
\hline \hline
0.5              & 1.65                   & 0.63                 & 61.5       & 1.6        & $4\!\times\!957^{3} =3517$\\
1                & 1.75                   & 0.81                 & 61.5       & 5          & $4\!\times\!479^{3} = \ \ 440.61$        \\
2                & 2.33                   & 0.52                  & 61.3       & 12        & $4\!\times\!239^{3} = \ \ \ \ 54.81$      \\
4               & 6.27                    & 0.72                 & 61.3      & 20         & $4\!\times\!118^{3}  = \ \ \ \ \ \ 6.57 $       \\
5               & 6.33                    & 0.69                 & 61.3       & 24          & $4\!\times\!95^{3} \ \ = \ \ \ \ \ \ 3.43 $       \\
8               & 11.73                   & 2.37                 & 55.2       & 32          & $4\!\times\!58^{3} \ \ = \ \ \ \ \ \ 0.78 $       \\
16               & 17.92                   & 5.52                & 45.7        & 40         & $4\!\times\!28^{3} \ \ = \ \ \ \ \ \ 0.09$        \\  \hline
\end{tabular}
%}
% \end{center}
% %\vspace{-1.0\baselineskip}

% %\vspace{-1\baselineskip}
\end{minipage}
%
\hfill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[t]{.05\linewidth}
\end{minipage}
\begin{minipage}[t]{.4\linewidth}
% \hfill
% \parbox{.5\columnwidth}{
\centering
\caption{\small Keypoint localization error, for training all three keypoints' radii simultaneously in one network and separately in three networks:  
$\bar{\epsilon}$
mean ($\mu_{\{sim|sep\}}$)  and standard deviation ($\sigma_{\{sim|sep\}}$)
for radial voting schemes.
\label{tab:NoofNets}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{tab-NumberofNetworks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \begin{center}
%\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{r|cc|cc}
% \cline{2-7}
% \multicolumn{1}{l}{} &
% \multicolumn{6}{c}{$\epsilon$ [mm]} \\ 
% \cline{4-9}
\multicolumn{1}{c}{} &
\multicolumn{4}{c}{$\bar{\epsilon}$ [mm]} \\
\cline{2-5}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{simultaneously}    & \multicolumn{2}{c}{separately} \\[-5pt]
% \cline{3-3} 
 \multicolumn{1}{c}{}
& \multicolumn{1}{c}{$\mu_{sim}$} & \multicolumn{1}{c}{$\sigma_{sim}$}
& \multicolumn{1}{c}{$\mu_{sep}$} & \multicolumn{1}{c}{$\sigma_{sep}$}\\ \hline \hline
ape & 1.7 & 0.9 & {\bf 1.3} & {\bf 0.7} \\ 
driller & 2.6 & 1.4 & {\bf 2.2} & {\bf 1.0} \\
eggbox & 2.5 & 1.3 & {\bf 2.0} & {\bf 0.7}\\ 
 \hline
\end{tabular}
%} % \resizebox
% \end{center}
% %\vspace{-0.7\baselineskip}
% %\vspace{-2\baselineskip}
% \end{table}
% %\vspace{-1 cm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\end{table}

==> tab-LINEMOD+OcclusionLINEMOD-2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
%\resizebox{\columnwidth}{!}{%
%   \resizebox{.75\columnwidth}{!}{%
\caption{\small LINEMOD and Occlusion LINEMOD accuracy results.
% Non-symmetric objects are evaluated with ADD, and
% symmetric objects
% (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
\label{tab:LINEMOD+OccLINEMOD}
}
\begin{tabular}{llcc}
\cline{3-4}
\multicolumn{2}{c}{} &
\multicolumn{2}{c}{ADD(s) [$\%$]} \\
\hline
Mode      & Method    
& LINEMOD & Occ. LINEMOD
\\\hline %\hline
&  SSD6D~\cite{kehl2017ssd} & 9.1 & - \\ % \cline{2-4}
& Oberweger~\cite{oberweger2018making}  & - & 27.1 \\% \cline{2-4} 
& Hu et al.~\cite{hu2019segmentation} & - & 30.4 \\% \cline{2-4} 
& Pix2Pose~\cite{park2019pix2pose}  & 72.4  & 32.0 \\% \cline{2-4} 
& DPOD~\cite{zakharov2019dpod}      & 83.0 & 32.8 \\% \cline{2-4} 
& PVNet~\cite{pvnet}      & 86.3 & 40.8 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-7}{*}{RGB}
%   \end{rotate}
& DeepIM~\cite{li2018deepim} & 88.6 & - \\ %\cline{2-4}
& PPRN~\cite{trabelsi2021ppn}    & 93.9     & 58.4 \\
& SO-Pose~\cite{di2021so}  & 96.0  & 62.3 \\\hline%\hline
 & YOLO6D~\cite{yolo6d}      & 56.0 & 6.4  \\%\cline{2-4} 
 & SSD6D+ref~\cite{kehl2017ssd} & 34.1 & 27.5 \\%\cline{2-4} 
                              
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & - & 24.9 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 95.2 & 47.3 \\\hline%\hline
& DenseFusion~\cite{wang2019densefusion}        & 94.3 &  - \\%\cline{2-4} 
& PVN3D~\cite{PVN3d}      & 99.4  & 63.2 \\%\cline{2-4} 
& PR-GCN~\cite{zhou2021pr}          & 99.6  & 65.0 \\
& FFB6D~\cite{he2021ffb6d}& {\bf 99.7}  & 66.2 \\
& RCVPose     & 99.4 & 70.2 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 99.7} & {\bf 71.1}\\ \hline
\end{tabular}
%} % \resizebox
\end{center}
% \vspace{-0.5\baselineskip}
% 
% \vspace{-1\baselineskip}
\end{table}

==> tab-LINEMOD+OcclusionLINEMOD.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\begin{center}
\resizebox{\columnwidth}{!}{%
%   \resizebox{.75\columnwidth}{!}{%
\begin{tabular}{c|c|c|c}
\cline{3-4}
\multicolumn{2}{c}{} &
\multicolumn{2}{c}{ADD(s) [$\%$]} \\
\hline
Mode      & Method    
& LINEMOD & Occ. LINEMOD
\\\hline \hline
&  SSD6D~\cite{kehl2017ssd} & 9.1 & - \\ \cline{2-4}
& Oberweger~\cite{oberweger2018making}  & - & 27.1 \\\cline{2-4} 
& Hu et al.~\cite{hu2019segmentation} & - & 30.4 \\\cline{2-4} 
& Pix2Pose~\cite{park2019pix2pose}  & 72.4  & 32.0 \\\cline{2-4} 
& DPOD~\cite{zakharov2019dpod}      & 83.0 & 32.8 \\\cline{2-4} 
& PVNet~\cite{pvnet}      & 86.3 & 40.8 \\\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& DeepIM~\cite{li2018deepim} & 88.6 & - \\ \cline{2-4}
& PPRN~\cite{trabelsi2021ppn}    & 93.9     & 58.4 \\\hline\hline
 & YOLO6D~\cite{yolo6d}      & 56.0 & 6.4  \\\cline{2-4} 
 & SSD6D+ref~\cite{kehl2017ssd} & 34.1 & 27.5 \\\cline{2-4} 
                              
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & - & 24.9 \\\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 95.2 & 47.3 \\\hline\hline
& DenseFusion~\cite{wang2019densefusion}        & 94.3 &  - \\\cline{2-4} 
& PVN3D~\cite{PVN3d}      & 99.4  & 63.2 \\\cline{2-4} 
& RCVPose     & 99.4 & 70.2 \\\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 99.7} & {\bf 71.1}\\ \hline
\end{tabular}
} % \resizebox
\end{center}
%\vspace{-0.5 cm}
\caption{LINEMOD and Occlusion LINEMOD accuracy results.\label{tab:LINEMOD+OccLINEMOD}
% Non-symmetric objects are evaluated with ADD, and
% symmetric objects
% (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
}

\end{table}

==> tab-LINEMOD-2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
%\resizebox{\columnwidth}{!}{%
%   \resizebox{.75\columnwidth}{!}{%
\begin{tabular}{llcc}
\cline{3-4}
\multicolumn{2}{c}{} &
\multicolumn{2}{c}{ADD(s) [$\%$]} \\
\hline
Mode      & Method    
& LINEMOD & Occ. LINEMOD
\\\hline %\hline
&  SSD6D~\cite{kehl2017ssd} & 9.1 & - \\ % \cline{2-4}
& Oberweger~\cite{oberweger2018making}  & - & 27.1 \\% \cline{2-4} 
& Hu et al.~\cite{hu2019segmentation} & - & 30.4 \\% \cline{2-4} 
& Pix2Pose~\cite{park2019pix2pose}  & 72.4  & 32.0 \\% \cline{2-4} 
& DPOD~\cite{zakharov2019dpod}      & 83.0 & 32.8 \\% \cline{2-4} 
& PVNet~\cite{pvnet}      & 86.3 & 40.8 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-7}{*}{RGB}
%   \end{rotate}
& DeepIM~\cite{li2018deepim} & 88.6 & - \\ %\cline{2-4}
& PPRN~\cite{trabelsi2021ppn}    & 93.9     & 58.4 \\
& SO-Pose~\cite{di2021so}  & 96.0  & 62.3 \\\hline%\hline
 & YOLO6D~\cite{yolo6d}      & 56.0 & 6.4  \\%\cline{2-4} 
 & SSD6D+ref~\cite{kehl2017ssd} & 34.1 & 27.5 \\%\cline{2-4} 
                              
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & - & 24.9 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 95.2 & 47.3 \\\hline%\hline
& DenseFusion~\cite{wang2019densefusion}        & 94.3 &  - \\%\cline{2-4} 
& PVN3D~\cite{PVN3d}      & 99.4  & 63.2 \\%\cline{2-4} 
& PR-GCN~\cite{zhou2021pr}          & 99.6  & 65.0 \\
& FFB6D~\cite{he2021ffb6d}& {\bf 99.7}  & 66.2 \\
& RCVPose     & 99.4 & 70.2 \\%\cline{2-4} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 99.7} & {\bf 71.1}\\ \hline
\end{tabular}
%} % \resizebox
\end{center}
%\vspace{-0.5\baselineskip}
\caption{LINEMOD and Occlusion LINEMOD accuracy results.\label{tab:LINEMOD+OccLINEMOD}
% Non-symmetric objects are evaluated with ADD, and
% symmetric objects
% (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
}
%\vspace{-1\baselineskip}
\end{table}

==> tab-ResnetVariation.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc|}
\cline{2-11}
\multirow{3}{*}{}             & \multicolumn{10}{c|}{Backbones (5 skip   connections)}                                                                                            \\ \cline{2-11} 
                              & \multicolumn{2}{c|}{Res-18} & \multicolumn{2}{c|}{Res-34} & \multicolumn{2}{c|}{Res-50} & \multicolumn{2}{c|}{Res-101} & \multicolumn{2}{c|}{Res-152} \\ \cline{2-11} 
                              & $\mu$       & $\sigma$      & $\mu$       & $\sigma$      & $\mu$       & $\sigma$      & $\mu$       & $\sigma$       & $\mu$       & $\sigma$       \\ \cline{2-11} \cline{2-11}\hline
\multicolumn{1}{|c|}{ape}     & 1.8         & 0.8           & 1.8         & 0.7           & 1.8         & 0.7           & 1.7         & 0.7            & 1.7         & 0.6            \\ \hline
\multicolumn{1}{|c|}{driller} & 2.7         & 0.8           & 2.7         & 0.8           & 2.6         & 0.6           & 2.7         & 0.7            & 2.5         & 0.5            \\ \hline
\multicolumn{1}{|c|}{eggbox}  & 2.4         & 1.2           & 2.4         & 1.1           & 2.3         & 1.1           & 2.2         & 1.1            & 2.1         & 0.8            \\ \hline
\end{tabular}
} % \resizebox
\caption{ResNet Backbone Accuracies: Deeper ResNet made minor improvment to the radial estimaiton. The unit is in mm}
\end{table}

==> tab-VotingTable3D-BBox.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\begin{center}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{r|c|cc|cc|cc}
% \cline{2-7}
% \multicolumn{1}{l}{} &
% \multicolumn{6}{c}{$\epsilon$ [mm]} \\ 
\cline{3-8}
\multicolumn{2}{c}{} &
\multicolumn{6}{c}{$\bar{\epsilon}$ [mm]} \\
 %  \cline{3-8}
\multicolumn{2}{l}{} & \multicolumn{2}{c}{vector}                & \multicolumn{2}{c}{offset}                    & \multicolumn{2}{c}{ radial}               \\[-5pt]
\cline{2-2} 
 \multicolumn{1}{c}{}
 &
 \multicolumn{1}{c|}{$\bar{r}$ [mm]}
&
\multicolumn{1}{c}{$\mu_v$} & \multicolumn{1}{c}{$\sigma_v$} & \multicolumn{1}{|c}{$\mu_o$} & \multicolumn{1}{c|}{$\sigma_o$} & \multicolumn{1}{c}{$\mu_r$} & \multicolumn{1}{c}{$\sigma_r$} \\ \hline \hline
 ape & 142.1 & 12.5 & 7.6 & 10.4 & 5.3 & {\bf 1.8} & {\bf 0.8} \\ \hline
driller & 318.8 & 11.3 &  8.2 &  9.5 &  3.5 &  {\bf 2.7} &  {\bf 0.8} \\ \hline
eggbox & 197.3 & 13.7 &  8.5 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ 
 \hline
% \cline{2-8}
%    & 13.7 &  8.5 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ \hline
\end{tabular}
} % \resizebox
\end{center}
\caption{Dispersed keypoint estimation error:  
$\bar{\epsilon}$
mean ($\mu_{\{v|o|r\}}$)  and standard deviation ($\sigma_{\{v|o|r\}}$)
for 3 voting schemes,
with 
$\bar{r}$
= mean distance of keypoints to object centroid}
\label{tab:KEE-BBox}
%\vspace{-1\baselineskip}
\end{table}


==> tab-VotingTable3D-FPS-BBox-rev1.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{r|c|c|cc|cc|cc|cc}
% \cline{2-7}
% \multicolumn{1}{l}{} &
% \multicolumn{6}{c}{$\epsilon$ [mm]} \\ 
% \cline{4-9}
\multicolumn{3}{c}{} &
\multicolumn{8}{c}{$\bar{\epsilon}$ [mm]} \\
\cline{4-11}
\multicolumn{3}{l}{} & \multicolumn{2}{c}{vector(Cartesian 3Q)}    & \multicolumn{2}{c}{vector(Spherical 2Q)}                & \multicolumn{2}{c}{offset}                    & \multicolumn{2}{c}{ radial}               \\[-5pt]
% \cline{3-3} 
 \multicolumn{2}{c}{}
 &
 \multicolumn{1}{c|}{$\bar{r}$ [mm]}
&
\multicolumn{1}{c}{$\mu_{v3}$} & \multicolumn{1}{c}{$\sigma_{v3}$} & \multicolumn{1}{|c}{$\mu_{v2}$} & \multicolumn{1}{c|}{$\sigma_{v2}$} & \multicolumn{1}{|c}{$\mu_{o}$} & \multicolumn{1}{c|}{$\sigma_{o}$} & \multicolumn{1}{c}{$\mu_r$} & \multicolumn{1}{c}{$\sigma_r$} \\ \hline \hline
ape & 
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{surface}}} 
& 61.2 & 10.0 & 5.8 & 5.6 & 2.4 & 5.8 & 2.6 & {\bf 1.3} & {\bf 0.7} \\ 
% \hline
% \cline{2-8}
 % & 12.5 & 7.6 & 10.4 & 5.3 & {\bf 1.8} & {\bf 0.8} \\ \hline
 % & 1 (GT) &  &  &  &  &  &  \\ \cline{2-8}
driller & & 129.4 & 10.0 & 2.3 & 5.3 & 2.5 & 6.5 & 4.7 & {\bf 2.2} & {\bf 1.0} \\ % \hline
% \cline{2-8}
%   & 11.3 &  8.2 &  9.5 &  3.5 &  {\bf 2.7} &  {\bf 0.8} \\ \hline
eggbox & & 82.5 & 11.8 & 5.3& 4.9 & 1.9 & 5.2 & 2.7 & {\bf 2.0} & {\bf 0.7}\\ 
 \hline
% \cline{2-8}
%    & 13.7 &  8.5 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ \hline

 ape & 
 % \multirow{3}{*}{disperse}
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{disperse}}} 
 & 142.1 & 12.5 & 7.6 & 5.7 & 2.5 & 10.4 & 5.3 & {\bf 1.8} & {\bf 0.8} \\ 
 % \hline
driller & & 318.8 & 11.3 &  8.2 & 5.2 & 2.6 &  9.5 &  3.5 &  {\bf 2.7} &  {\bf 0.8} \\ 
% \hline
eggbox & & 197.3 & 13.7 &  8.5 & 7.2 & 3.4 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ 
 \hline
% \cline{2-8}
%    & 13.7 &  8.5 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ \hline
\end{tabular}
} % \resizebox
\end{center}
%\vspace{-1\baselineskip}
\caption{Keypoint localization error, for surface and disperse keypoints:  
$\bar{\epsilon}$
mean ($\mu_{\{v|o|r\}}$)  and standard deviation ($\sigma_{\{v|o|r\}}$)
for 3 voting schemes,
$\bar{r}$
= mean keypoint distance to object centroid.}
\label{tab:KEE-FPS-BBox}
%\vspace{-1\baselineskip}
\end{table}
% \vspace{-1 cm}


==> tab-VotingTable3D-FPS.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{r|c|cc|cc|cc}
% \cline{2-7}
% \multicolumn{1}{l}{} &
% \multicolumn{6}{c}{$\epsilon$ [mm]} \\ 
\cline{3-8}
\multicolumn{2}{c}{} &
\multicolumn{6}{c}{$\bar{\epsilon}$ [mm]} \\
 %  \cline{3-8}
\multicolumn{2}{l}{} & \multicolumn{2}{c}{vector}                & \multicolumn{2}{c}{offset}                    & \multicolumn{2}{c}{ radial}               \\[-5pt]
\cline{2-2} 
 \multicolumn{1}{c}{}
 &
 \multicolumn{1}{c|}{$\bar{r}$ [mm]}
&
\multicolumn{1}{c}{$\mu_v$} & \multicolumn{1}{c}{$\sigma_v$} & \multicolumn{1}{|c}{$\mu_o$} & \multicolumn{1}{c|}{$\sigma_o$} & \multicolumn{1}{c}{$\mu_r$} & \multicolumn{1}{c}{$\sigma_r$} \\ \hline \hline
ape & 61.2 & 10.0 & 5.8 & 5.8 & 2.6 & {\bf 1.3} & {\bf 0.7} \\ \hline
% \cline{2-8}
 % & 12.5 & 7.6 & 10.4 & 5.3 & {\bf 1.8} & {\bf 0.8} \\ \hline
 % & 1 (GT) &  &  &  &  &  &  \\ \cline{2-8}
driller & 129.4 & 10.0 & 2.3 & 6.5 & 4.7 & {\bf 2.2} & {\bf 1.0} \\ \hline
% \cline{2-8}
%   & 11.3 &  8.2 &  9.5 &  3.5 &  {\bf 2.7} &  {\bf 0.8} \\ \hline
eggbox & 82.5 & 11.8 & 5.3 & 5.2 & 2.7 & {\bf 2.0} & {\bf 0.7}\\ 
 \hline
% \cline{2-8}
%    & 13.7 &  8.5 &  11.4 &  4.7 &  {\bf 2.4} &  {\bf 1.2} \\ \hline
\end{tabular}
} % \resizebox
\end{center}
\caption{Surface keypoint estimation error:  $\bar{\epsilon}$ mean ($\mu_{\{v|o|r\}}$)  and standard deviation ($\sigma_{\{v|o|r\}}$)
for 3 voting schemes,
with 
$\bar{r}$
= mean distance of keypoints to object centroid}
\label{tab:KEE-FPS}
%\vspace{-1\baselineskip}
\end{table}

==> tab-YCB-2.tex <==

\begin{table}[ht]
\begin{center}
%\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{clcc}
\hline  
\begin{tabular}{c} %\vspace{-3 pt} 
Refine? 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt} 
Method 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt}
%   \overline{\mbox{ADD(s)} [$\%$]}
\mbox{ADD(s)} [$\%$]
\end{tabular} 
&
\begin{tabular}{c} %\vspace{-3 pt}
% \overline{\mbox{AUC} [$\%$]} 
\mbox{AUC} [$\%$]
\end{tabular} 
\\ [3pt]
\hline%\hline
\multicolumn{1}{c}{{}}                          & {PoseCNN~\cite{posecnn} } 
& 59.9 &  75.8
\\ %\cline{2-4} 
\multicolumn{1}{c}{{}}                              & {DF (per-pixel)~\cite{wang2019densefusion}}  
& 82.9 & 91.2
\\%  \cline{2-4} 
\multicolumn{1}{c}{{}} & {PVN3D~\cite{PVN3d}}
& 91.8 & 95.5
\\ % \cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{No}}     & RCVPose                              
 & \textbf{95.2} & \textbf{96.6}
 \\ \hline%  \hline
\multicolumn{1}{c}{}                          & PoseCNN~\cite{posecnn} 
& 85.4 & 93.0
\\ % \cline{2-4} 
 \multicolumn{1}{c}{}                          & {DF (iterative)~\cite{wang2019densefusion}} 
 & 86.1 & 93.2
 \\ %\cline{2-4} 
\multicolumn{1}{c}{}                          & {PVN3D~\cite{PVN3d}+ICP} 
& 92.3 & 96.1
\\ %\cline{2-4} 
 \multicolumn{1}{c}{\multirow{-4}{*}{Yes}}     & RCVPose+ICP                         
 & \textbf{95.9} & \textbf{97.2}
 \\ \hline
\end{tabular}
%\end{adjustbox}
%\vspace{-0.5\baselineskip}
%\vspace{+0.1\baselineskip}
\caption{YCB-Video accuracy results.\label{tab:ycbvideo}}
\end{center}
%\vspace{-2\baselineskip}
\end{table}

==> tab-YCB-3.tex <==

\begin{table}[ht]
\begin{center}
\caption{\small YCB-Video accuracy results.
\label{tab:ycbvideo}
} 
%\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lrcccccc}
\cline{3-8} %\vspace{-3 pt}
% \hline  
% \begin{tabular}{c} \vspace{-3 pt} 
% Refine? 
% \end{tabular} 
% & 
% \begin{tabular}{c} \vspace{-3 pt} 
% Method 
% \end{tabular} 
& 
&
\multicolumn{2}{c}{\mbox{ADD(s)} [$\%$]}
& & 
% \overline{\mbox{AUC} [$\%$]} 
\multicolumn{3}{c}{\mbox{AUC} [$\%$]}
\\ [3pt]
\cline{1-2}
Method & refine? & no & yes && no && yes \\
\hline%\hline
% \multicolumn{1}{c}{{}}                          & 
{PoseCNN~\cite{posecnn} } 
& & 59.9 & 85.4 && 75.8 && 93.0
\\ %\cline{2-4} 
% \multicolumn{1}{c}{{}}                              & 
{DF (per-pixel)~\cite{wang2019densefusion}}  
& & 82.9 & 86.1 && 91.2 && 93.2
\\%  \cline{2-4} 
% \multicolumn{1}{c}{{}} & 
{SO-Pose~\cite{di2021so}}
& & 56.8 & - && 90.9 && - 
\\
{PVN3D~\cite{PVN3d}}
& & 91.8 & 92.3 && 95.5 && 96.1
\\ % \cline{2-4} 
{PR-GCN~\cite{zhou2021pr}}
& & - & - && 95.8 && -
\\
%  \multicolumn{1}{c}{\multirow{-4}{*}{No}}     & 
{FFB6D~\cite{he2021ffb6d}}
& & 92.7 & 93.1 && \textbf{96.6} && 97.0 
\\
 RCVPose                              
&  & \textbf{95.2} & \textbf{95.9} && \textbf{96.6} && \textbf{97.2}
 \\ \hline%  \hline
% \multicolumn{1}{c}{}                          & PoseCNN~\cite{posecnn} 
% & 85.4 & 93.0
% \\ % \cline{2-4} 
%  \multicolumn{1}{c}{}                          & {DF (iterative)~\cite{wang2019densefusion}} 
%  & 86.1 & 93.2
%  \\ %\cline{2-4} 
% \multicolumn{1}{c}{}                          & {PVN3D~\cite{PVN3d}+ICP} 
% & 92.3 & 96.1
% \\ %\cline{2-4} 
%  \multicolumn{1}{c}{\multirow{-4}{*}{Yes}}     & RCVPose+ICP                         
%  & \textbf{95.9} & \textbf{97.2}
%  \\ \hline
\end{tabular}
%\end{adjustbox}
%\vspace{-0.5\baselineskip}
% \vspace{+0.1\baselineskip}
% 
\end{center}
% \vspace{-2\baselineskip}
\end{table}

==> tab-YCB.tex <==

\begin{table}[]
\begin{center}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c}
\hline  
\begin{tabular}{c} %\vspace{-3 pt} 
Refine? 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt} 
Method 
\end{tabular} 
& 
\begin{tabular}{c} %\vspace{-3 pt}
%   \overline{\mbox{ADD(s)} [$\%$]}
\mbox{ADD(s)} [$\%$]
\end{tabular} 
&
\begin{tabular}{c} %\vspace{-3 pt}
% \overline{\mbox{AUC} [$\%$]} 
\mbox{AUC} [$\%$]
\end{tabular} 
\\ [3pt]
\hline\hline
\multicolumn{1}{c|}{{}}                          & {PoseCNN~\cite{posecnn} } 
& 59.9 &  75.8
\\ \cline{2-4} 
\multicolumn{1}{c|}{{}}                              & {DF (per-pixel)~\cite{wang2019densefusion}}  
& 82.9 & 91.2
\\ \cline{2-4} 
\multicolumn{1}{c|}{{}} & {PVN3D~\cite{PVN3d}}
& 91.8 & 95.5
\\ \cline{2-4} 
 \multicolumn{1}{c|}{\multirow{-4}{*}{No}}     & RCVPose                              
 & \textbf{95.2} & \textbf{96.6}
 \\ \hline \hline
\multicolumn{1}{c|}{}                          & PoseCNN~\cite{posecnn} 
& 85.4 & 93.0
\\ \cline{2-4} 
 \multicolumn{1}{c|}{}                          & {DF (iterative)~\cite{wang2019densefusion}} 
 & 86.1 & 93.2
 \\ \cline{2-4} 
\multicolumn{1}{c|}{}                          & {PVN3D~\cite{PVN3d}+ICP} 
& 92.3 & 96.1
\\ \cline{2-4} 
 \multicolumn{1}{c|}{\multirow{-4}{*}{Yes}}     & RCVPose+ICP                         
 & \textbf{95.9} & \textbf{97.2}
 \\ \hline
\end{tabular}
\end{adjustbox}
%\vspace{-0.5\baselineskip}
\caption{YCB-Video accuracy results\label{tab:ycbvideo}}
\end{center}
%\vspace{-2\baselineskip}
\end{table}

==> tab-keypointsSelection.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{c|c|c|c}
\cline{2-4}
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Number of Keypoints} \\ %   \cline{2-4} 
\multicolumn{1}{c|}{}        & 3           & 4          & 8       \\ \hline \hline
\multicolumn{1}{c|}{ape}                       & 61.3        & 60.9       & 61.3        \\ \hline
\multicolumn{1}{c|}{driller}                   & 78.8        & 78.6       & 78.8       \\ \hline
\multicolumn{1}{c|}{eggbox }                   & 82.3        & 82.6       & 82.3          \\ \hline
\end{tabular}
\end{center}
\caption{Accuracy w.r.t. Number of Keypoints}
\label{tab:AccVsNKeypts}
\end{table}

==> tab-linemod.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\begin{center}
\resizebox{.75\columnwidth}{!}{%
\begin{tabular}{c|c|c}
\hline
\begin{tabular}{c} %\vspace{-3 pt} 
Mode 
\end{tabular} 
      & 
\begin{tabular}{c} %\vspace{-3 pt} 
Method 
\end{tabular} 
      &  
\begin{tabular}{c} %\vspace{-3 pt} 
   \overline{\mbox{ADD(s) [$\%$]}}
    ADD(s) [$\%$]
\end{tabular}       
\\[3pt]
\hline \hline 
                                & SSD6D+ref~\cite{kehl2017ssd}  & 9.1 \\\cline{2-3}  
                                & Pix2Pose~\cite{park2019pix2pose} & 72.4 \\\cline{2-3}  
                                & DPOD~\cite{zakharov2019dpod} & 83.0 \\\cline{2-3}  
                                & PVNet~\cite{pvnet}       & 86.3 \\\cline{2-3}  
                                & PPRN~\cite{trabelsi2021ppn}       & 93.9 \\\cline{2-3}  
\multirow{-6}{*}{RGB}           & DeepIM~\cite{li2018deepim}    & 88.6 \\\hline\hline
                                & YOLO6D~\cite{yolo6d}     & 56.0  \\\cline{2-3} 
\multirow{-2}{*}{RGB}
                                & SSD6D+ref~\cite{kehl2017ssd}   & 34.1 \\\cline{2-3}  
\multirow{-2}{*}{+D ref}      & DPOD+ref~\cite{zakharov2019dpod}  & 95.2 \\\hline \hline
                                & DenseFusion~\cite{wang2019densefusion}    & 94.3 \\\cline{2-3}  
                                & PVN3D~\cite{PVN3d}      & 99.4 \\\cline{2-3}  
                                & FFB6d~\cite{he2021ffb6d}&
                                & RCVPose                  & 99.4 \\\cline{2-3}  
\multirow{-4}{*}{RGB-D}         & RCVPose+ICP              & {\bf 99.7}\\ \hline
\end{tabular}
} % \resizebox
\end{center}
\caption{LINEMOD accuracy results}
%   \vspace{-1.5\baselineskip}
\label{tab:Linemod}
\end{table}

==> tab-occlinemod-full-1.tex <==
\begin{comment}
\begin{table*}[t]
%   \resizebox{\columnwidth}{!}{%
%   \resizebox{\pagewidth}{!}{%
\begin{center}
\caption{Occlusion LINEMOD Accuracy Results.
Non-symmetric objects are evaluated with ADD, and
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD-s%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics. 
}
%   \begin{tabularx}
%\vspace{1.25 cm} \\
\begin{tabular}
{r|c|c|c|c|c|c|c|c|c|c|c|c|c}
%   \cline{1-1} \\
\multicolumn{1}{c|}{Object}      &
%   Object &
\begin{rotate}{60} 
YOLO6D 
\end{rotate} & 
\begin{rotate}{60} 
SSD6D+ref 
\end{rotate}
& 
\begin{rotate}{60} 
PoseCNN 
\end{rotate}
& 
\begin{rotate}{60} 
Oberweger 
\end{rotate}
& 
\begin{rotate}{60} 
 Hu et al. 
\end{rotate}
& 
\begin{rotate}{60} 
 Pix2Pose
\end{rotate}
& 
\begin{rotate}{60} 
 DPOD
\end{rotate}
& 
\begin{rotate}{60} 
 PVNet
\end{rotate}
& 
\begin{rotate}{60} 
 DPOD+ref 
\end{rotate}
& 
\begin{rotate}{60} 
 PPRN 
\end{rotate}
& 
\begin{rotate}{60} 
 PVN3D 
\end{rotate}
& 
\begin{rotate}{60} 
 PoseCNN+ICP 
\end{rotate}
&  
\begin{rotate}{60} 
 RCVPose
\end{rotate}
\\ \hline \hline
ape         & -                                 & -                                    & 9.6                                  & 12.1                                   & 17.6                                   & 22                                    & -                               & 15.8                              & -                    & -              & 33.9                               & 76.2                & 60.3 \\ \hline
can         & -                                 & -                                    & 45.2                                 & 39.9                                   & 53.9                                   & 44.7                                  & -                               & 63.3                               & -                    & -               & 88.6                               & 87.4               & 92.5  \\ \hline
cat         & -                                 & -                                    & 0.93                                 & 8.2                                    & 3.3                                    & 22.7                                  & -                               & 16.7                             & -                    & -                & 39.1                               & 52.2              & 50.2   \\ \hline
driller     & -                                 & -                                    & 41.4                                 & 45.2                                   & 62.4                                   & 44.7                                  & -                               & 25.2                            & -                    & -                & 78.4                               & 90.3              &78.2   \\ \hline
duck        & -                                 & -                                    & 19.6                                 & 17.2                                   & 19.2                                   & 15                                    & -                               & 65.6                            & -                    & -                 & 41.9                               & 77.7             & 52.1   \\ \hline
eggbox      & -                                 & -                                    & 22                                   & 22.1                                   & 25.9                                   & 25.2                                  & -                               & 50.2                              & -                    & -                 & 80.9                               & 72.2             & 81.2    \\ \hline
glue        & -                                 & -                                    & 38.5                                 & 35.8                                   & 39.6                                   & 32.4                                  & -                               & 49.6                              & -                    & -                & 68.1                               & 76.7              & 72.0   \\ \hline
holepuncher & -                                 & -                                    & 22.1                                 & 36                                     & 21.3                                   & 49.5                                  & -                               & 39.7                              & -                    & -                 & 74.7                               & 91.4             & 75.2   \\ \hline \hline
mean        & 6.4                               & 27.5                                   & 24.9                                 & 27                                     & 27                                     & 32                                    & 32.8                             & 40.8                              & 47.2                 & 58.4              & 63.2                               & 78               & 70.2    \\ \hline
%   \end{tabularx}
\end{tabular}
\end{center}
\\
\caption{Occlusion LINEMOD Leaderboard}
\label{tab:OccLinemod}
%   } % \resizebox
\end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\begin{center}
%   \resizebox{2\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\cline{3-10}
\multicolumn{2}{c|}{}
&
\multicolumn{8}{c|}{Object}  \\ [3pt]
\cline{1-2}
\cline{11-11}
%   \hline
Mode      & Method     & ape  & can  & cat  & driller & duck & eggbox$^{*}$ & glue$^{*}$ & holepuncher &
\begin{tabular}{c}%\vspace{-3 pt} 
\overline{\mbox{ADD(s)}} [$\%$] 
\end{tabular}
\\\hline \hline
                                & Oberweger~\cite{oberweger2018making}  & 12.1 & 39.9 & 8.2  & 45.2    & 17.2 & 22.1   & 35.8 & 36.0        & 27.1 \\\cline{2-11} 
                                & Hu et al.~\cite{hu2019segmentation}  & 17.6 & 53.9 & 3.3  & 62.4    & 19.2 & 25.9   & 39.6 & 21.3        & 30.4 \\\cline{2-11} 
                                & Pix2Pose~\cite{park2019pix2pose}   & 22.0 & 44.7 & 22.7 & 44.7    & 15.0 & 25.2   & 32.4 & 49.5        & 32.0 \\\cline{2-11} 
                                & DPOD~\cite{zakharov2019dpod}       & -  & -  & -  & -     & -  & -    & -  & -         & 32.8 \\\cline{2-11} 
                                & PVNet~\cite{pvnet}      & 15.8 & 63.3 & 16.7 & 25.2    & \textbf{65.7} & 50.2   & 49.6 & 39.7        & 40.8 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& PPRN~\cite{trabelsi2021ppn}       & -  & -  & -  & -     & -  & -    & -  & -         & 58.4 \\\hline\hline
                                & YOLO6D~\cite{yolo6d}     & -  & -  & -  & -     & -  & -    & -  & -         & 6.4  \\\cline{2-11} 
                                & SSD6D+ref~\cite{kehl2017ssd}  & -  & -  & -  & -     & -  & -    & -  & -         & 27.5 \\\cline{2-11} 
                               
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}    & 9.6  & 45.2 & 0.9  & 41.4    & 19.6 & 22.0   & 38.5 & 22.1        & 24.9 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & -  & -  & -  & -     & -  & -    & -  & -         & 47.3 \\\hline\hline
                                & PVN3D~\cite{PVN3d}      & 33.9 & 88.6 & 39.1 & 78.4   & 41.9 & 80.9   & 68.1 & 74.7        & 63.2 \\\cline{2-11} 
                                & RCVPose     & 60.3 & 92.5 & 50.2 & 78.2    & 52.1 & 81.2   & 72.1  & 75.2        & 70.2 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP & {\bf 61.3} & {\bf 93} & {\bf 51.2} & {\bf 78.8}   & 53.4 & {\bf 82.3}   & {\bf 72.9} & {\bf 75.8}        & {\bf 71.1}\\ \hline
\end{tabular}
\end{center}
%   } % \resizebox

\label{tab:OccLinemod}
\end{table*}

==> tab-occlinemod.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\resizebox{.75\columnwidth}{!}{%
\begin{tabular}{c|c|c}
\hline
Mode      & Method    
&
ADD(s) [$\%$] 
\\\hline \hline
                                & Oberweger~\cite{oberweger2018making}  & 27.1 \\\cline{2-3} 
                                & Hu et al.~\cite{hu2019segmentation} & 30.4 \\\cline{2-3} 
                                & Pix2Pose~\cite{park2019pix2pose}  & 32.0 \\\cline{2-3} 
                                & DPOD~\cite{zakharov2019dpod}      & 32.8 \\\cline{2-3} 
                                & PVNet~\cite{pvnet}     & 40.8 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& PPRN~\cite{trabelsi2021ppn}         & 58.4 \\\hline\hline
                                & YOLO6D~\cite{yolo6d}      & 6.4  \\\cline{2-3} 
                                & SSD6D+ref~\cite{kehl2017ssd} & 27.5 \\\cline{2-3} 
                               
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}      & 24.9 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & 47.3 \\\hline\hline
                                & PVN3D~\cite{PVN3d}        & 63.2 \\\cline{2-3} 
                                & RCVPose      & 70.2 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{RGB-D}  
%   \end{rotate}
& RCVPose+ICP  & {\bf 71.1}\\ \hline
\end{tabular}
} % \resizebox
\end{center}
\caption{Occlusion LINEMOD accuracy results.
% Non-symmetric objects are evaluated with ADD, and
% symmetric objects
% (annotated with~$^{*}$) are evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics. 
}
\label{tab:OccLinemod}
\end{table}

==> tab-test.tex <==
\begin{table}[!htb]
    \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{}
      \centering
        \begin{tabular}{ll}
            1 & 2
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{}
        \begin{tabular}{ll}
            3 & 4
        \end{tabular}
    \end{minipage} 
\end{table}
